Leveraging LLMs for Dynamic IoT Systems Generation through Mixed-Initiative Interaction

IoT systems face significant challenges in adapting to user needs, which are often under-specified and evolve with changing environmental contexts. To address these complexities, users should be able to explore possibilities, while IoT systems must learn and support users in the process of providing proper services, e.g., to serve novel experiences. The IoT-Together paradigm aims to meet this demand through the Mixed-Initiative Interaction (MII) paradigm that facilitates a collaborative synergy between users and IoT systems, enabling the co-creation of intelligent and adaptive solutions that are precisely aligned with user-defined goals. This work advances IoT-Together by integrating Large Language Models (LLMs) into its architecture. Our approach enables intelligent goal interpretation through a multi-pass dialogue framework and dynamic service generation at runtime according to user needs. To demonstrate the efficacy of our methodology, we design and implement the system in the context of a smart city tourism case study. We evaluate the system's performance using agent-based simulation and user studies. Results indicate efficient and accurate service identification and high adaptation quality. The empirical evidence indicates that the integration of Large Language Models (LLMs) into IoT architectures can significantly enhance the architectural adaptability of the system while ensuring real-world usability.

==> sections/expt.tex <==

\textbf{Representative Conversation Analysis:}
To illustrate the effectiveness of our three-pass dialogue structure in service identification, let's analyze a representative conversation from our user study that demonstrates the system's ability to handle complex, multi-faceted queries:

\begin{quote}
\textbf{User:} What are various landmarks or interesting places that I can visit in the city? Also, I am currently located at IIIT Hyderabad, Gachibowli. I also want to know, how do I get there? Like what all convenient ways of travel can I take, such that my travel is hassel-free? Also let me, know, any convenient nearby places where I can stay, or where my relatives can stay when they are visiting.

\textbf{System:} Hello there! I'm your friendly Hyderabad City Guide, here to help you explore the vibrant city of Hyderabad. It's a wonderful place with a rich history and plenty of interesting landmarks. To get started, could you tell me a bit about your interests? Are you more inclined towards historical sites, nature, shopping, or perhaps food? Also, how much time do you have to explore today?

\textbf{User:} We are inclinded towards historical sites or monuments, however we like food and nature too. When me and my relatives go around to visit places, we often want food stops and all. It is not just today, we have the entire week to travel and explore. Also, since I will be travelling with my family, I would prefer private vehicles. However, I would want to accomodate my family in some nice hotel or some place in the city. And I would want to first reach there, and then we can carry on our trip from there.

\textbf{System:} That sounds like a fantastic plan! Exploring historical sites while enjoying local cuisine and the beauty of nature will surely make for a memorable trip. Let me suggest some must-visit historical landmarks in Hyderabad that you can explore throughout the week...
[System provides detailed recommendations for historical sites, nature spots, food stops, travel options, and accommodation suggestions]

\textbf{User:} I think a few of these places of stay may be in localities that are too expensive. Could we have a more budget-friendly accomodation? Also, I will be having a lot of relatives over. So booking a lot of cabs for them may not be ideal. Could you perhaps suggest some private bus service for us?

\textbf{System:} Based on our conversation, I've identified these services and parameters:

�� travel\_options:
   • preferred\_mode: private\_transport
   • destination: [multiple locations]
�� historical\_info:
   • site\_name: [Charminar, Golconda Fort, Mecca Masjid, Chowmahalla Palace, Qutb Shahi Tombs]
�� restaurant\_finder:
   • group\_size: 4

Does this accurately reflect what you're looking for?

\textbf{User:} Yes
\end{quote}

This conversation demonstrates the three-pass dialogue structure:

1. \textbf{First Pass - Context Gathering:}
   \begin{itemize}
      \item Identified user's location (IIIT Hyderabad, Gachibowli)
      \item Probed for interests in historical sites, nature, shopping, or food
      \item Inquired about time availability and travel preferences
   \end{itemize}

2. \textbf{Second Pass - Goal Refinement:}
   The user specified:
   \begin{itemize}
      \item Interest in historical sites and monuments
      \item Secondary interests in food and nature
      \item Week-long exploration timeframe
      \item Preference for private vehicle transport
      \item Need for family accommodation
   \end{itemize}

3. \textbf{Third Pass - Service Identification:}
   The system identified and parameterized three key services:
   \begin{itemize}
      \item \texttt{travel\_options}: 
         \begin{itemize}
            \item preferred\_mode: private\_transport
         \end{itemize}
      \item \texttt{historical\_info}:
         \begin{itemize}
            \item site\_name: [Charminar, Golconda Fort, Mecca Masjid, Chowmahalla Palace, Qutb Shahi Tombs]
         \end{itemize}
      \item \texttt{restaurant\_finder}:
         \begin{itemize}
            \item group\_size: 4
         \end{itemize}
   \end{itemize}

This conversation demonstrates the system's ability to handle complex, multi-faceted queries and progressively refine them into concrete service parameters. The user confirmed the accuracy of these identified services and parameters, validating the effectiveness of our approach in understanding and decomposing user requirements.

